QCD for Collider Physics

These lectures are directed at a level suitable for graduate students in experimental and theoretical High Energy Physics. They are intended to give an introduction to the theory and phenomenology of quantum chromodynamics (QCD) as it is used in collider physics applications. The aim is to bring the reader to a level where informed decisions can be made concerning different approaches and their uncertainties. The material is divided into four main areas: 1) fundamentals, 2) perturbative QCD, 3) soft QCD, and 4) Monte Carlo event generators.

==> Makefile <==
DOC = eshep-skands
BIB = eshep-skands
#SUBDIRS = jimmyplots plots_pythia6_pub #lhceffects lhc_parp90

#all: subdirs $(DOC).pdf
all: $(DOC).pdf

subdirs:
	for dir in $(SUBDIRS); do \
	  $(MAKE) -C $$dir; \
	done

$(DOC).pdf: $(DOC).tex $(BIB).bib subdirs
	if test ! -e $(DOC).aux; then pdflatex $(DOC); fi
	bibtex $(DOC) || rm $(DOC).aux
	while true; do pdflatex $(DOC); \
      if grep -i rerun $(DOC).log; then true; else break; fi; done

dist: $(DOC).dep
	bundledoc --config=$(HOME)/local/texmf/tex/latex/bundledoc/tetex.cfg  $(DOC).dep

clean:
	rm -f $(DOC).pdf *.aux $(DOC).toc $(DOC).bbl $(DOC).blg $(DOC).log $(DOC).out; \
	for dir in $(SUBDIRS); do \
	  rm -f $$dir/*pdf; \
	done


